Mitigating False Predictions In Unreasonable Body Regions

Despite considerable strides in developing deep learning models for 3D medical image segmentation, the challenge of effectively generalizing across diverse image distributions persists. While domain generalization is acknowledged as vital for robust application in clinical settings, the challenges stemming from training with a limited Field of View (FOV) remain unaddressed. This limitation leads to false predictions when applied to body regions beyond the FOV of the training data. In response to this problem, we propose a novel loss function that penalizes predictions in implausible body regions, applicable in both single-dataset and multi-dataset training schemes. It is realized with a Body Part Regression model that generates axial slice positional scores. Through comprehensive evaluation using a test set featuring varying FOVs, our approach demonstrates remarkable improvements in generalization capabilities. It effectively mitigates false positive tumor predictions up to 85% and significantly enhances overall segmentation performance.

==> boundaries_table.tex <==
    \centering
        \caption{List of all MSD 5-fold cross-validation Dice scores for the MultiTalent networks trained with different valid boundaries between $\mu$ and $\mu\pm6\sigma$ to determine the best boundaries for each class. The networks were trained for 1000 epochs to reduce compute overhead and without a Gaussian boundary weighting to find the best-fitting boundaries for each class. }\label{all_boundaries_Dice_scores}
    \begin{adjustbox}{width = 0.8\textwidth}
    \begin{tabular}{cccccccccccccc}
    \toprule
        \multicolumn{2}{c}{class} & \multicolumn{2}{c}{mean slice scores} &\multicolumn{10}{c}{Dice for different offsets to the mean slice scores }\\
        \cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-14}
         no & name & minimum & maximum& $0\sigma$ & $0.5\sigma$ & $1\sigma$ & $1.5\sigma$ & $2\sigma$ & $2.5\sigma$ & $3\sigma$ & $4\sigma$ & $5\sigma$ & $6\sigma$\\
        \midrule
        1 & liver & $33.09\pm3.31$ & $52.73\pm1.88$  & 95.72 & 95.80 & 95.82 & 95.79 & \textcolor{blue}{95.89} & 95.84 & 95.85 & 95.84 & 95.89 & 95.81 \\ 
        2 & liver tumor & $39.4\pm5.46$ & $48.49\pm4.39$  & \textcolor{blue}{64.25} & 62.55 & 63.55 & 62.79 & 63.15 & 62.82 & 64.23 & 61.99 & 62.13 & 62.59 \\ 
        3 & lung tumor & $61.25\pm4.5$ & $64.55\pm5.15$  & 67.23 & 67.88 & 65.95 & 67.54 & 67.35 & 65.43 & 66.14 & 68.02 & \textcolor{blue}{68.60} & 66.68 \\ 
         4 & pancreas & $34.34\pm1.96$ & $44.1\pm1.68$  & 79.86 & 79.97 & 79.97 & 80.01 & \textcolor{blue}{80.03} & 79.85 & 79.90 & 79.78 & 79.81 & 80.02 \\ 
        5 & pancreas cancer & $37.67\pm2.74$ & $40.38\pm2.88$  & 55.29 & 54.51 & 55.07 & \textcolor{blue}{55.84} & 55.62 & 55.32 & 55.76 & 55.11 & 55.27 & 55.56 \\ 
        6 & hepatic vessel & $36.14\pm4.09$ & $51.61\pm1.74$  & 63.76 & \textcolor{blue}{64.17} & 64.14 & 63.92 & 63.76 & 64.07 & 63.89 & 64.00 & 64.01 & 63.89 \\ 
        7 & liver cancer & $40.74\pm4.66$ & $47.65\pm3.96$ & 70.90 & \textcolor{blue}{70.95} & 70.27 & 70.71 & 70.92 & 70.78 & 70.55 & 69.75 & 69.93 & 70.66 \\ 
        8 & spleen & $39.87\pm2.34$ & $50.37\pm1.93$  & 96.13 & 96.07 & 96.14 & 96.26 & 96.29 & 96.26 & 96.20 & 96.23 & \textcolor{blue}{96.30} & 96.27 \\ 
        9 & colon cancer & $24.03\pm8.83$ & $29.49\pm9.29$  & 52.96 & 52.41 & 51.91 & 51.21 & \textcolor{blue}{53.10} & 51.31 & 50.96 & 52.42 & 51.04 & 49.79 \\ 
        % 10 & spleen & $38.91\pm2.72$ & $50.24\pm2.05$ & 91.63 & \textcolor{blue}{92.83} & 91.88 & 92.60 & 91.57 & 92.08 & 92.64 & 92.58 & 92.42 & 91.32 \\ 
        % 11 & right kidney & $30.61\pm2.18$ & $42.89\pm2.14$ & 88.79 & 89.27 & 89.38 & 89.25 & 88.30 & 89.42 & 89.71 & 89.61 & \textcolor{blue}{89.77} & 89.73 \\ 
        % 12 & left kidney & $31.5\pm2.42$ & $43.84\pm1.62$ & 88.77 & 89.19 & 88.83 & 88.54 & 87.39 & 89.13 & 88.85 & 88.91 & 88.87 & \textcolor{blue}{89.49} \\ 
        % 13 & gallbladder & $37.71\pm3.11$ & $42.56\pm2.3$ & 67.33 & 67.13 & 68.91 & 68.43 & 65.37 & \textcolor{blue}{69.44} & 69.39 & 68.97 & 69.32 & 69.28 \\ 
        % 14 & esophagus & $47.83\pm0.97$ & $56.83\pm4.94$ & 78.42 & 78.74 & 78.21 & 78.25 & 77.86 & \textcolor{blue}{79.33} & 79.17 & 78.88 & 79.06 & 78.93 \\ 
        % 15 & liver & $31.63\pm3.3$ & $53.09\pm1.87$ & 95.15 & 95.46 & 95.67 & 95.72 & 95.37 & \textcolor{blue}{95.78} & 95.75 & 95.71 & 95.75 & 95.65 \\ 
        % 16 & stomach & $37.11\pm2.63$ & $50.62\pm2.05$ & 87.62 & 88.67 & 89.32 & 88.86 & \textcolor{blue}{90.08} & 89.31 & 90.01 & 89.84 & 88.86 & 88.99 \\ 
        % 17 & aorta & $29.34\pm1.92$ & $56.52\pm3.97$  & 86.89 & 87.06 & 87.33 & 88.14 & 88.66 & 89.45 & 89.86 & \textcolor{blue}{90.36} & 90.32 & 90.13 \\ 
        % 18 & vena cava inferior & $28.74\pm2.08$ & $54.23\pm1.32$ & 85.03 & 85.37 & \textcolor{blue}{85.50} & 85.28 & 84.87 & 85.31 & 85.24 & 84.91 & 85.29 & 85.40 \\ 
        % 19 & portal \& splenic vein & $39.7\pm1.24$ & $46.68\pm0.9$  & 75.52 & 75.94 & 75.66 & 75.55 & \textcolor{blue}{77.00} & 75.96 & 75.79 & 75.77 & 75.83 & 75.60 \\ 
        % 20 & pancreas & $34.76\pm2.05$ & $44.81\pm1.05$ & 83.16 & 83.56 & 83.49 & 83.80 & 83.47 & 83.63 & \textcolor{blue}{83.92} & 83.51 & 83.83 & 83.88 \\ 
        % 21 & right adrenal gland & $41.76\pm1.57$ & $45.87\pm1.18$ & 68.81 & 70.87 & 69.22 & 69.90 & \textcolor{blue}{71.31} & 70.02 & 70.80 & 70.08 & 71.09 & 69.47 \\ 
        % 22 & left adrenal gland & $40.36\pm1.09$ & $45.39\pm1.24$ & 68.36 & 68.46 & 69.58 & 68.83 & 65.70 & 69.86 & 69.20 & 69.32 & 69.36 & \textcolor{blue}{69.93} \\ 
        % 23 & spleen & $38.47\pm2.88$ & $49.86\pm1.75$  & 92.17 & 92.43 & 92.15 & 92.53 & 91.97 & 92.24 & 92.53 & \textcolor{blue}{92.54} & 92.21 & 91.84 \\ 
        % 24 & left kidney & $31.72\pm2.07$ & $44.06\pm1.64$  & 90.77 & 90.88 & 90.71 & 90.49 & 90.33 & \textcolor{blue}{90.94} & 90.77 & 90.60 & 90.69 & 90.90 \\ 
        % 25 & gallbladder & $38.01\pm3.36$ & $43.18\pm3.13$  & 75.28 & 75.89 & 75.99 & 75.97 & 73.20 & \textcolor{blue}{77.06} & 76.93 & 75.87 & 76.17 & 76.13 \\ 
        % 26 & esophagus & $45.72\pm3.03$ & $54.15\pm3.75$ & 69.23 & 69.16 & 69.30 & 69.37 & 68.88 & 69.61 & 69.37 & 69.74 & \textcolor{blue}{69.92} & 69.37 \\ 
        % 27 & liver & $32.53\pm3.33$ & $52.75\pm1.83$ & 93.47 & 93.69 & 93.81 & 93.89 & \textcolor{blue}{93.94} & 93.91 & 93.86 & 93.88 & 93.80 & 93.79 \\ 
        % 28 & stomach & $37.9\pm3.63$ & $50.22\pm2.01$ & 86.87 & 88.24 & 88.35 & 88.27 & 89.14 & 88.59 & 88.35 & \textcolor{blue}{89.21} & 88.47 & 88.51 \\ 
        % 29 & pancreas & $34.93\pm1.95$ & $44.64\pm1.11$  & 82.30 & 82.61 & 82.48 & 82.63 & 82.59 & 82.56 & 82.61 & 82.47 & 82.62 & \textcolor{blue}{82.64} \\ 
        % 30 & duodenum & $32.0\pm2.07$ & $42.82\pm1.99$ & 71.38 & 71.61 & 71.14 & 71.54 & 71.01 & 71.76 & 71.88 & 71.47 & \textcolor{blue}{71.96} & 71.60 \\ 
        % 31 & left lung & $45.57\pm1.64$ & $75.02\pm1.17$ & 95.79 & 95.79 & 95.64 & \textcolor{blue}{95.86} & 95.70 & 95.84 & 95.81 & 95.72 & 95.80 & 95.79 \\ 
        % 32 & right lung & $45.41\pm1.54$ & $75.02\pm1.62$ & 96.48 & 96.54 & 96.30 & 96.52 & 96.36 & \textcolor{blue}{96.60} & 96.45 & 96.53 & 96.58 & 96.52 \\ 
        % 33 & heart & $48.83\pm1.67$ & $62.85\pm1.22$ & 93.26 & 93.22 & 93.37 & 93.39 & \textcolor{blue}{93.43} & 93.26 & 93.29 & 93.37 & 93.21 & 93.34 \\ 
        % 34 & esophagus & $48.0\pm1.75$ & $78.02\pm1.14$  & 79.47 & 79.51 & 79.62 & 79.60 & 79.69 & 79.51 & 79.67 & 79.70 & 79.46 & \textcolor{blue}{79.83} \\ 
        % 35 & bronchies & $57.92\pm1.67$ & $77.82\pm1.62$ & 83.17 & 82.99 & 83.22 & 83.02 & \textcolor{blue}{83.37} & 83.09 & 83.21 & 83.21 & 83.22 & 83.22 \\ 
        % 36 & spinal cord nerve & $34.05\pm3.55$ & $88.33\pm1.56$ & 89.06 & 89.18 & 89.33 & 89.44 & \textcolor{blue}{90.30} & 89.39 & 89.50 & 89.57 & 89.63 & 89.38 \\ 
        % 37 & esophagus & $47.9\pm0.89$ & $75.85\pm1.32$  & 82.11 & 81.85 & 82.26 & 82.33 & 81.97 & \textcolor{blue}{82.68} & 82.35 & 82.54 & 82.52 & 82.41 \\ 
        % 38 & heart & $49.06\pm1.55$ & $60.54\pm1.01$  & 93.54 & 93.83 & 93.81 & \textcolor{blue}{93.97} & 93.77 & 93.86 & 93.86 & 93.80 & 93.67 & 93.94 \\ 
        % 39 & trachea & $61.86\pm1.01$ & $75.87\pm1.34$ & 89.58 & 89.49 & 89.58 & 89.65 & 89.53 & \textcolor{blue}{89.89} & 89.89 & 89.70 & 89.43 & 89.75 \\ 
        % 40 & aorta & $43.67\pm1.31$ & $69.15\pm0.94$ & 92.51 & 92.62 & 92.78 & 92.88 & 92.66 & 92.90 & 92.89 & \textcolor{blue}{92.99} & 92.72 & 92.91 \\ 
        % 41 & pancreas & $35.39\pm1.6$ & $45.05\pm1.08$ & \textcolor{blue}{82.24} & 82.20 & 82.20 & 82.13 & 81.67 & 82.19 & 82.16 & 82.03 & 82.14 & 82.17 \\ 
        % 42 & both kidneys & $30.09\pm4.2$ & $44.48\pm1.53$ & 92.85 & 93.09 & 92.59 & 92.13 & 91.31 & 90.80 & 92.60 & 93.36 & 94.06 & \textcolor{blue}{94.85} \\ 
        % 43 & kidney tumor & $34.48\pm4.6$ & $39.91\pm3.82$ & 78.09 & 78.24 & 77.54 & 77.80 & \textcolor{blue}{79.11} & 78.45 & 77.70 & 77.08 & 77.72 & 77.78 \\ 
        % 44 & bladder & $6.77\pm0.99$ & $17.54\pm3.79$  & 89.32 & 89.21 & \textcolor{blue}{90.33} & 88.94 & 88.25 & 90.31 & 89.89 & 89.40 & 89.80 & 89.40 \\ 
        % 45 & uterus & $4.79\pm2.51$ & $18.73\pm3.15$ & 78.99 & 78.62 & 78.96 & \textcolor{blue}{79.07} & 78.56 & 78.94 & 78.22 & 78.08 & 78.56 & 78.89 \\ 
        % 46 & rectum & $2.93\pm2.48$ & $15.37\pm2.99$ & 74.05 & 73.95 & 73.91 & 73.57 & 74.28 & 74.03 & 73.63 & 74.48 & 74.34 & \textcolor{blue}{74.99} \\ 
        % 47 & small bowel & $14.79\pm3.47$ & $30.4\pm3.36$  & 54.46 & 55.73 & 55.60 & 54.65 & \textcolor{blue}{55.76} & 53.10 & 54.38 & 53.77 & 52.85 & 52.09 \\
        % \midrule
        %  \multicolumn{2}{c}{mean} & & &81.23 & 81.44 & 81.42 & 81.42 & 81.27 & 81.53 & \textcolor{blue}{81.61} & 81.55 & 81.58 & 81.51 \\ 
        %  \multicolumn{2}{c}{std} & & &11.90 & 11.98 & 12.00 & 12.05 & 12.00 & 12.14 & 12.08 & 12.15 & 12.17 & 12.32 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    
